Semigroup algorithmic problems in metabelian groups

We consider semigroup algorithmic problems in finitely generated metabelian groups. Our paper focuses on three decision problems introduced by Choffrut and Karhum\"{a}ki (2005): the Identity Problem (does a semigroup contain a neutral element?), the Group Problem (is a semigroup a group?) and the Inverse Problem (does a semigroup contain the inverse of a generator?). We show that all three problems are decidable for finitely generated sub-semigroups of finitely generated metabelian groups. In particular, we establish a correspondence between polynomial semirings and sub-semigroups of metabelian groups using an interaction of graph theory, convex polytopes, algebraic geometry and number theory. Since the Semigroup Membership problem (does a semigroup contain a given element?) is known to be undecidable in finitely generated metabelian groups, our result completes the decidability characterization of semigroup algorithmic problems in metabelian groups.

==> dump.tex <==
\begin{lem}\label{lem:realtorat}
Condition~\emph{(LocInf)} of Theorem~\ref{thm:locglob} is equivalent to the following:

\begin{enumerate}[noitemsep]
    \item[2'.] \emph{\textbf{(LocInfRat):}}  For every $v \in \Qns$, there exists $\bff_{v} \in \mM$, such that 
    \begin{enumerate}[noitemsep]
        \item[(a')] $\init_{v}\left(\bff_{v}\right) \in \ApK$.
        %\item $\left(O_{v} \cup J\right) \cap M_{I, v}(\bff_{v}) \neq \emptyset$.
        \item[(b')] Denote $I' \coloneqq M_{v}(I, \bff_{v}), J' \coloneqq O_{v} \cup J$.
        We have 
        \begin{equation}\label{eq:locvrat}
        \left(O_{w} \cup J'\right) \cap M_{w}(I', \init_{v}(\bff_{v})) \neq \emptyset \quad \text{ for every $w \in \Rns$}.
        \end{equation}
    \end{enumerate}
\end{enumerate}
\end{lem}
\begin{proof}
    The direction (LocInf)$\implies$(LocInfRat) is immediate.
    For the direction (LocInfRat)$\implies$(LocInf), suppose (LocInfRat) holds.
    Let $\bg_1 = (g_{11}, \ldots, g_{iK}), \ldots, \bg_m = (g_{m1}, \ldots, g_{mK})$ be a super Gr\"{o}bner basis of $\mM$.
    Given an irrational $\tv \in \Rns$, there exists a close enough rational $v \in \Qns$ \red{justify} such that $\init_v(g_{ji}) = \init_{\tv}(g_{ji})$ for all $j, i$, and $v_i \tv_i > 0$ whenever $\tv_i \neq 0$.

    By assumption (LocInfRat) there exists $\bff \in \mM$ such that, writing $\beta_i \coloneqq - \deg_v(f_i)$ we have $\init_{v, \bbeta}(\bff) \in \ApK$.
    Put
    \[
    \tbeta_i \coloneqq - \deg_{\tv}(\init_v f_i),
    \]
    so that $\max_{1 \leq i \leq K}\{\deg_{\tv}(\init_v f_i) + \tbeta_i\} = 0$ and $\init_{\tv, \tbbeta}(\init_{v, \bbeta}(\bff)) \in \ApK$.
    Let $\prec_0$ be an arbitrary term order on the monomials of $\R[\oX]$.
    Define $\delta \in \{-1, 1\}^n$ be letting $\delta_i = 1$ if $v_i \geq 0$ and $\delta_i = -1$ if $v_i < 0$.
    Let $|v|$ and $|\tv|$ denote the elements of $\R^n$ with $|v|_i = |v_i|$ and $|\tv|_i = |\tv_i|$.
    For $u, u' \in \Zp^n$ and $i, i' \in \{1, \ldots, K\}$, put $X_1^{\delta_1 u_1} \cdots X_n^{\delta_n u_n} e_i \prec X_1^{\delta_1 u'_1} \cdots X_n^{\delta_n u'_n} e_{i'}$ if
    \begin{enumerate}[noitemsep, label = (\arabic*)]
        \item $\beta_i + u \cdot |v| < \beta_{i'} + u' \cdot |v|$, or
        \item $\beta_i + u \cdot |v| = \beta_{i'} + u' \cdot |v|$ and $\tbeta_i + u \cdot |\tv| < \tbeta_{i'} + u' \cdot |\tv|$, or
        \item $\beta_i + u \cdot |v| = \beta_{i'} + u' \cdot |v|$, $\tbeta_i + u \cdot |\tv| = \tbeta_{i'} + u' \cdot |\tv|$ and $\oX^u e_i \prec_0 \oX^{u'} e_{i'}$.
    \end{enumerate}
    This defines a term order on the monomials of $\R[X_1^{\delta_1}, \ldots, X_n^{\delta_n}]^K$.
    \red{Justify} we have $w \in \Z^n$ and $p_j \in \R[\oX]$ such that $\oX^w \bff, \oX^w p_j \bg_j \in \R[X_1^{\delta_1}, \ldots, X_n^{\delta_n}]^K$, $\bff = \sum_{i = 1}^m p_j \bg_j$ and
    \[
    \init_{\prec}(\oX^w \bff) = \max_{\prec} \{\init_{\prec}(\oX^w p_j \bg_j) \mid j = 1, \ldots, m\}.
    \]
    Let
    \[
    A \coloneqq \left\{j \in \{1, \ldots, m\} \;\middle|\; \deg_{v, \bbeta}(\bff) = \deg_{v, \bbeta}(p_j \bg_j)\} \right\},
    \]
    we obtain 
    \[
    \sum_{j \in A} \init_{v, \beta}(p_j \bg_j) = \init_{v, \beta}(\bff) \in \ApK
    \]
    by property (1) of the term order $\prec$.

    Furthermore, letting
    \[
    B \coloneqq \left\{j \in A \;\middle|\; \deg_{\tv, \tbbeta}(\init_{v, \beta}(p_j \bg_{j}))\} = 0 = \deg_{\tv, \tbbeta}(\init_{v, \bbeta} (\bff)) \right\},
    \]
    we have
    \[
    \sum_{j \in B} \init_{\tv, \tbbeta}(\init_{v, \bbeta}(p_j \bg_j)) = \init_{\tv, \tbbeta}(\init_{v, \bbeta}(\bff)) \in \ApK
    \]
    by property (2) of the term order $\prec$.

    Let $i \in \{1, \ldots, K\}$.
    Put $B_i \coloneqq \{j \in B \mid \init_{\tv, \tbbeta}(\init_{v, \bbeta}(p_j \bg_j))_i \neq 0\}$.
    Then
    \begin{equation}\label{eq:starstar}
    \sum_{j \in B_i} \init_{\tv}(\init_{v}(p_{j})) \init_{\tv}(g_{ji}) = \sum_{j \in B_i} \init_{\tv}(\init_{v}(p_j g_{ji})) =  \init_{\tv}(\init_v(f_i)) \in \A^+
    \end{equation}
    by the fact that $\init_v(g_{ji}) = \init_{\tv}(g_{ji})$.
    
    Consider $\bg \coloneqq \sum_{j \in B} \init_v(p_j) \bg_j \in \mM$.
    We will show that $\bff_{tv} \coloneqq \bg$ satisfies conditions~(a) and (b) for $\tv$.
    
    The polynomials $h_j \coloneqq \init_v(p_j)$ satisfy $h_j = \init_v(h_j)$.
    Note that
    \[
    \init_{\tv}(h_j g_{ji}) = \init_{\tv}(h_j) \init_{\tv}(g_{ji}) = \init_{\tv}(h_j) \init_{\tv}(\init_v(g_{ji})) = \init_{\tv}(\init_v(h_j g_{ji})).
    \]
    Since $B$ consists of those $j \in A$ such that the maximum of $\deg_{\tv, \tbbeta}(\init_{v, \bbeta}(h_j \bg_{j}))$ is obtained, we also have
    \begin{align*}
        \max_{j \in B} \deg_{\tv}(h_j g_{ji}) = \max_{j \in B} \deg_{\tv}(\init_v(h_j g_{ji})) = \max_{j \in A} \deg_{\tv}(\init_{v, \bbeta}(h_j g_{j})_i) = \deg_{\tv}(\init_{v, \bbeta}(f_i)) = - \tbeta_i.
    \end{align*}
    As $B_i \coloneqq \{j \in B \mid \deg_{\tv}(\init_{\tv}(\init_{v}(p_j)g_{ji})) = - \tbeta_i\}$, it then follows from \eqref{eq:starstar} that
    \[
        \init_{\tv}(\bg)_i = \init_{\tv, \tbbeta}(\bg)_i = \sum_{j \in B_i} \init_{\tv}(\init_{v}(p_{j})) \init_{\tv}(g_{ji}) \in \A^+.
    \]
    We have thus shown condition~(a).
    For condition~(b), notice
    \[
    \init_{\tv, \tbbeta}(\bg) = \init_{\tv, \tbbeta}(\init_{v}(\bff)) \in \ApK,
    \]
    so $M_{tv}(I, \bg) = M_{tv}(I, \init_{v}(\bff))$.
\end{proof}

\begin{lem}\label{lem:condtoprime}
Condition~(2) of Theorem~\ref{thm:locglob} is equivalent to the following:

\begin{enumerate}[noitemsep]
    \item[(2')]  For every $P \in \mP$, there exists $\bff_{v_P} \in \mM$ as well as some $\balpha_{P, Q}$, %satisfying 
    %\begin{equation}
    %    \left(O_{v_P} \cup J\right) \cap \{i \in I \mid \alpha_{P, Q, i} = \min_{j \in J} \alpha_{P, Q, j}\} \neq \emptyset,
    %\end{equation}
    such that 
    \begin{enumerate}[noitemsep]
        \item[(a')] $\init_{v_P, \balpha_{P, Q}}\left(\bff_{v_P}\right) \in \ApK$.
        \item[(b')] Denote $I'' \coloneqq \{i \in I \mid \alpha_{P, Q, i} = \min_{j \in I} \alpha_{P, Q, j}\}, J'' \coloneqq \left(O_{v_P} \cup J\right)$.
        We have 
        \[
        \left(O_{w} \cup J''\right) \cap M_{w}(I'', \init_{v_P, \balpha_{P, Q}}(\bff_{v_P})) \neq \emptyset \quad \text{ for every $w \in \Rns$}.
        \]
    \end{enumerate}
\end{enumerate}
\end{lem}
\begin{proof}
    $(2) \implies (2')$:
    Suppose Condition~(2) of Theorem~\ref{thm:locglob} is true.
    Then in particular it holds for the vector $v_P \in \Rns$.
    So there exists $\bff_{v_P} \in \mM$, such that $\init_{v_P}\left(\bff_{v_P}\right) \in \ApK$ and
    \begin{equation}\label{eq:cond58}
        \left(O_{w} \cup J'\right) \cap M_{w}(M_{v_P}(I, \bff_{v_P}), \init_{v_P}(\bff_{v_P})) \neq \emptyset \quad \text{ for every $w \in \Rns$}.
    \end{equation}
    Define $\balpha = \left(- \deg_{v_P}(f_{v_P, 1}), \ldots, - \deg_{v_P}(f_{v_P, K}) \right) \in \R^K$. It is well defined since $f_{v_P, i} \neq 0, i = 1, \ldots, K$.
    
    Then $\init_{v_P, \balpha}\left(\bff_{v_P}\right) = \init_{v_P}\left(\bff_{v_P}\right) \in \ApK$ and 
    \[
    I' = M_{v_P}(I, \bff_{v_P}) = \{i \in I \mid \alpha_{i} = \min_{j \in I} \alpha_{j}\} = \{i \in I \mid \alpha_{P, Q, i} = \min_{j \in I} \alpha_{P, Q, j}\} = I''
    \]
    by Lemma~\ref{lem:eqPQ}.
    Hence
    \[
        \left(O_{w} \cup J''\right) \cap M_{w}(I'', \init_{v_P, \balpha_{P, Q}}(\bff_{v_P})) \neq \emptyset \quad \text{ for every $w \in \Rns$}
    \]
    follows from $J' = J''$ and Equation~\eqref{eq:cond58}.

    $(2') \implies (2)$: 
    Suppose Condition~(2') is true, we want to show that Condition~(2) of Theorem~\ref{thm:locglob} hold for every $v \in \Rns$.
    Take any $v \in \Rns$, let $P \in \mP$ be such that $v \Rpp \in P$.
    Then there exists $Q \in \mL$ and $\balpha_{P, Q}$ satisfying conditions~(a') and (b').
    By the definition of $P$, there exists $\balpha \in \R^K$ such that $(v, \balpha) \Rpp \in Q$.
    Then by Lemma~\ref{lem:eqPQ}, we have $\init_{v, \balpha}\left(\bff_{v_P}\right) = \init_{v_P, \balpha_{P, Q}}\left(\bff_{v_P}\right) \in \ApK$ \red{wrong},
    so
    \[
    \deg_{v}(f_{v_P, 1}) + \alpha_1 = \cdots = \deg_{v}(f_{v_P, K}) + \alpha_K
    \]
    and $\init_{v}\left(\bff_{v_P}\right) = \init_{v, \balpha}\left(\bff_{v_P}\right) \in \ApK$ \red{add lemma or observation that justifies this}.
    Therefore,
    \[
    I' = M_{v_P}(I, \bff_{v_P}) = \{i \in I \mid \alpha_{i} = \min_{j \in I} \alpha_{j}\} = \{i \in I \mid \alpha_{P, Q, i} = \min_{j \in I} \alpha_{P, Q, j}\} = I''.
    \]
    Furthermore, $O_{v} = O_{v_P}$, so $J' = J''$.
    We have
    \[
    \left(O_{w} \cup J'\right) \cap M_{w}(I', \init_{v}(\bff_{v_P})) = \left(O_{w} \cup J''\right) \cap M_{w}(I'', \init_{v_P, \balpha_{P, Q}}\left(\bff_{v_P}\right)) \neq \emptyset
    \]
    by Condition~(b').
    Therefore, Condition~(2) of Theorem~\ref{thm:locglob} is satisfied by $\bff_{v} \coloneqq \bff_{v_P}$.
\end{proof}

\begin{lem}\label{lem:in0gen}
    $\init_{v, \balpha}^0(\mM)$ is generated by $\init_{v, \balpha}^0(\bg_1), \ldots, \init_{v, \balpha}^0(\bg_m)$.
\end{lem}
\begin{proof}
    By \cite[Lemma~2.1]{einsiedler2003does}, the set
    \[
    \init_{v, \balpha}(\mM) \coloneqq \left\{\init_{v, \balpha}(\bff) \;\middle|\; \bff \in \mM \right\}
    \]
    is generated by $\init_{v, \balpha}(\bg_1), \ldots, \init_{v, \balpha}(\bg_m)$.
    
    On one hand, take any $\bff^0 \in \init_{v, \balpha}^0(\mM)$, we show $\bff^0$ is in the $\A_{n-1}$-module generated by $\init_{v, \balpha}^0(\bg_1), \ldots, \init_{v, \balpha}^0(\bg_m)$.
    By \cite[Lemma~2.1]{einsiedler2003does}, there exists $\bff \in \mM$ such that $\bff^0 = X_n^{- d(\bff)} \cdot \init_{v, \balpha}(\bff)$.
    Write
    \[
    \init_{v, \balpha}(\bff) = \sum_{i = 1}^m p_i \cdot \init_{v, \balpha}(\bg_i),
    \]
    then 
    \[
    \bff^0 = X_n^{- d(\bff)} \cdot \init_{v, \balpha}(\bff) = \sum_{i = 1}^m p_i X_n^{- d(\bff)} \cdot \init_{v, \balpha}(\bg_i) = \sum_{i = 1}^m p_i \cdot \init_{v, \balpha}^0(\bg_i).
    \]
    So $\bff^0$ is in the $\A_{n-1}$-module generated by $\init_{v, \balpha}^0(\bg_1), \ldots, \init_{v, \balpha}^0(\bg_m)$.

    On the other hand, take any element
    \[
    \bff^0 \coloneqq \sum_{i = 1}^m q_i \cdot \init_{v, \balpha}^0(\bg_i)
    \]
    in the $\A_{n-1}$-module generated by $\init_{v, \balpha}^0(\bg_1), \ldots, \init_{v, \balpha}^0(\bg_m)$, we show that it is in $\init_{v, \balpha}^0(\mM)$.
    Since
    \[
    \bff^0 = \sum_{i = 1}^m q_i X_n^{d(\bg_i)} \cdot \init_{v, \balpha}(\bg_i)
    \]
    is also in the $\A_{n-1}$-module generated by $\init_{v, \balpha}(\bg_1), \ldots, \init_{v, \balpha}(\bg_m)$.
    Therefore there exists $\bff \in \mM$ such that $\bff^0 = \init_{v, \balpha}(\bff)$.
    But since $\bff^0$ is already in $\A_{n-1}^K$, we have $\bff^0 = \init_{v, \balpha}^0(\bff) \in \init_{v, \balpha}^0(\mM)$.

    We conclude that $\init_{v, \balpha}^0(\mM)$ is exactly the $\A_{n-1}$-module generated by $\init_{v, \balpha}^0(\bg_1), \ldots, \init_{v, \balpha}^0(\bg_m)$.
\end{proof}

\begin{prop}\label{prop:shifttozero}
Condition~\emph{(LocInfShift)} of Proposition~\ref{prop:inftoshift} is equivalent to 
\begin{enumerate}[noitemsep]
    \item[(2'')] \emph{\textbf{(LocInfZero):}}  For every $v \in \Rns$, let $P \in \mP$ be the cell containing $v$. Assume after a change of coordinates $P$ is an open subset of $\langle e_1, \ldots, e_d \rangle^{\perp}$.
    Then there is some $\balpha \in \left(\sum_{i = d+1}^n \Z v_i\right) ^K$ \red{(highlight not R)} and $\bff^d \in \init_{v, \balpha}^d(\mM)$ satisfying
    \begin{enumerate}
        \item[(a'')] $\bff^d \in \left(\A_{d}^+\right)^K$.
        \item[(b1'')] We have
        \begin{equation}\label{eq:conddouble}
            \left(O_{v} \cup J\right) \cap \{i \in I \mid \alpha_{P, Q, i} = \min_{j \in I} \alpha_{P, Q, j}\} \neq \emptyset
        \end{equation}
        \item[(b2'')] Denote $I'' \coloneqq \{i \in I \mid \alpha_{v, i} = \min_{j \in I} \alpha_{v, j}\}, J'' \coloneqq \left(O_{v} \cup J\right)$, we have
        \begin{equation}\label{eq:conddouble2}
        \left(O_{u} \cup J''\right) \cap M_{u}(I'', \bff^d) \neq \emptyset \quad \text{ for every $u \in \left(\R^{d}\right)^*$}.
    \end{equation}
    \end{enumerate}
\end{enumerate}
\end{prop}
\begin{proof}
    $(2') \implies (2'')$:
    Suppose Condition~(2') of Proposition~\ref{prop:inftoshift} is true.
    Fix $P \in \mP$, then Condition~(2') of Proposition~\ref{prop:inftoshift} gives $\bff_{v_P} \in \mM$ and $\balpha_{P, Q}$ satisfying (a') and (b').
    After a change of variables, we can suppose $v_P = e_n$.
    Write $\init_{v_P, \balpha_{P, Q}}\left(\bff_{v_P}\right) = X_n^{d} \cdot \bff$ with $\bff \in \init_{v_P, \balpha_{P, Q}}^0(\mM) \cap \left(\A_{n-1}^+\right)^K$.
    We will show that Condition~(2'') is satisfied by the same $\balpha_{P, Q}$ and this $\bff$.

    Take $w = v_P$ in Condition~(b'), we get 
    $
    \left(O_{v_P} \cup J\right) \cap M_{v_P}(I'', \init_{v_P, \balpha_{P, Q}}(\bff_{v_P})) \neq \emptyset
    $.
    Therefore 
    \[
    \left(O_{v_P} \cup J\right) \cap I'' \supseteq \left(O_{v_P} \cup J\right) \cap M_{v_P}(I'', \init_{v_P, \balpha_{P, Q}}(\bff_{v_P})) \neq \emptyset.
    \]
    So Condition~\eqref{eq:conddouble} is satisfied.

    We now deduce Condition~\eqref{eq:conddouble2}.
    By Lemma~\ref{lem:tweakinit}, there exists an open neighbourhood $U$ of $v_P \Rpp$ such that for every $(v_P + u)\Rpp \in U$,
    \begin{multline}\label{eq:Udouble}
    \init_{v_P + u}\left(\bff_{v_P}\right) = \init_{u}\left(\init_{v_P}(\bff_{v_P})\right), \; M_{v_P + u}(I, \bff) = M_{u}(M_{v_P}(I, \bff_{v_P}), \init_{v_P}(\bff_{v_P})), \\
    \text{ and } \; O_{v_P + u} = O_{v_P} \cup O_{u}.
    \end{multline}
    Fix a $u \in \left(\R^{n-1}\right)^*$. 
    By scaling $u$ by a small enough number we can indeed suppose $(v_P + u)\Rpp \in U$.
    We apply Condition~(b') to $w = v_P + u$.
    This yields $\left(O_{v_P + u} \cup J''\right) \cap M_{v_P + u}(I'', \init_{v_P, \balpha_{P, Q}}(\bff_{v_P})) \neq \emptyset$.
    Since $\init_{v_P, \balpha_{P, Q}}\left(\bff_{v_P}\right) \in \ApK$, we have $I'' = M_{v_P}(I, \bff_{v_P})$ and $\init_{v}\left(\bff_{v_P}\right) = \init_{v, \balpha}\left(\bff_{v_P}\right)$ as in the proof of Proposition~\ref{prop:inftoshift}.
    Hence,
    \begin{multline*}
    \left(O_{u} \cup J''\right) \cap M_{u}(I'', \bff) = \left(O_{u} \cup (O_{v_P} \cup J)\right) \cap M_{u}(I'', X_n^{d} \cdot \bff) \\
    = \left(O_{v_P + u} \cup (O_{v_P} \cup J)\right) \cap M_{u}(I'', \init_{v_P, \balpha_{P, Q}}(\bff_{v_P})) = \left(O_{v_P + u} \cup J''\right) \cap M_{u}(M_{v_P}(I, \bff_{v_P}), \init_{v_P}(\bff_{v_P}))\\
    = \left(O_{v_P + u} \cup J''\right) \cap M_{v_P + u}(I, \bff) \neq \emptyset.
    \end{multline*}
    This yields Condition~\eqref{eq:conddouble2}.

    $(2'') \implies (2')$:
    Suppose Condition~(2'') is true.
    Fix a $P \in \mP$, without loss of generality suppose $v_P = e_n$.
    Let $\balpha_{P, Q}$ and $\bff \in \init_{v_P, \balpha_{P, Q}}^0(\mM) \cap \left(\A_{n-1}^+\right)^K$ be as defined in Condition~(2'').
    By the definition of $\init_{v_P, \balpha_{P, Q}}^0(\mM)$, there exists $\bff_{v_P} \in \mM$ such that $\init_{v_P, \balpha_{P, Q}}(\bff_{v_P}) = X_n^d \cdot \bff$ \red{correct this}.
    We will show that Condition~(2') is satisfied by the same $\balpha_{P, Q}$ and this $\bff_{v_P} \in \mM$.

    Since $\bff \in \left(\A_{n-1}^+\right)^K$ we have $\init_{v_P, \balpha_{P, Q}}(\bff_{v_P}) = X_n^d \cdot \bff \in \ApK$, which yields Condition~(a').

    For Condition~(b'), we have as before $I'' = M_{v_P}(I, \bff_{v_P})$ and $\init_{v}\left(\bff_{v_P}\right) = \init_{v, \balpha}\left(\bff_{v_P}\right)$.
    Take any $w \in \Rns$.

    If $w \in v_P \Rpp$, then Condition~(b') is equivalent to $\left(O_{v_P} \cup J''\right) \cap I'' \neq \emptyset$, which follows from Equation~\eqref{eq:conddouble}.

    If $w \not\in v_P \Rpp$. Let $u \in \left(\R^{n-1}\right)^*$ be such that $w = u + \delta v_P$ for some $\delta \in \Rpp$.
    Then
    \begin{multline*}
    O_{w} \cup O_{v_P} = \{v \mid v \not\perp w \lor v \not\perp v_P\} = \{v \mid v \not\perp u + \delta v_P \lor v \not\perp v_P\} = \{v \mid \neg(v \perp u + \delta v_P \land v \perp v_P)\} \\
    = \{v \mid \neg(v \perp u \land v \perp v_P)\} = \{v \mid v \not\perp u \lor v \not\perp v_P\} = O_{u} \cup O_{v_P}
    \end{multline*}
    Hence,
    \begin{multline*}
        \left(O_{w} \cup J''\right) \cap M_{w}(I'', \init_{v_P, \balpha_{P, Q}}(\bff_{v_P})) = \left(O_{w} \cup O_{v_P} \cup J\right) \cap M_{w}(I'', X_n^d \cdot \bff) \\
        = \left(O_{u} \cup O_{v_P} \cup J\right) \cap M_{w}(I'', \bff) = \left(O_{u} \cup J''\right) \cap M_{u}(I'', \bff) \neq \emptyset.
    \end{multline*}
    This yields Condition~(b').
\end{proof}

\begin{lem}\label{lem:eqPQ}
    Let $Q \in \mL$. For $(v, \balpha) \Rpp \in Q$, we have
    \[
    \init_{v, \balpha}(\mM) = \init_{v_P, \balpha_{P, Q}}(\mM), \;\; \{i \in I \mid \alpha_{i} = \min_{j \in I} \alpha_{j}\} = \{i \in I \mid \alpha_{P, Q, i} = \min_{j \in I} \alpha_{P, Q, j}\}, \; \text{ and } \;\; O_{v} = O_{v_P}.
    \]
\end{lem}
\begin{proof}
    By \cite[Lemma~6.1]{einsiedler2003does}, when $(v, \balpha) \Rpp$ and $(v_P, \balpha_{P, Q}) \Rpp$ belong to the same element of $\mL_{\mM}$, we have $\init_{v, \balpha}(\mM) = \init_{v_P, \balpha_{P, Q}}(\mM)$.
    By definition of $\mL_I$, when $\balpha \Rpp$ and $\balpha_{P, Q} \Rpp$ belong to the same element of $\mL_I$, we have $\min_{j \in I} \alpha_{j}\} = \{i \in I \mid \alpha_{P, Q, i} = \min_{j \in I} \alpha_{P, Q, j}\}$.
    By definition of $\mL_O$, when $v \Rpp$ and $v_P \Rpp$ belong to the same element of $\mL_O$, we have $O_{v} = O_{v_P}$.

    Note that $\mL \coloneqq \mL_{\mM} \vee \mL'_I \vee \mL'_O$.
    Because $(v, \balpha) \Rpp$ and $(v_P, \balpha_{P, Q}) \Rpp$ belong to the same element of $\mL$, all three equations in the statement of the lemma are satisfied.
\end{proof}

Fix a pair $(v_P, \balpha_{P, Q}) \Rpp \in Q$.
Denote 
\[
\A_{n-1} \coloneqq \R[X_1^{\pm}, \ldots, X_{n-1}^{\pm}], \quad \A_{n-1}^+ \coloneqq \Rp[X_1^{\pm}, \ldots, X_{n-1}^{\pm}]^*.
\]
Using a suitable change of vectors we can even assume without loss of generality that $v_P \in e_n \Rpp$.
For $\bff \in \A^{K} \setminus \{0\}$, there exists a unique $d(\bff) \in \Z$ such that
\[
\init_{v_P, \balpha_{P, Q}}^0(\bff) \coloneqq X_n^{- d(\bff)} \init_{v_P, \balpha_{P, Q}}(\bff) \in \A_{n-1}^K.
\]
In fact, it suffices to take $d(\bff)$ to be $\deg_{v_P}(f_i)$ such that $\deg_{v_P}(f_i) + \alpha_i$ is largest among $i \in \{1, \ldots, K\}$.

\begin{proof}
Note that $\A = \R[X_1^{\pm}, \ldots, X_n^{\pm}]$. We use induction on $n$.
When $n = 0$, we do not have any degree constraints and the problem reduces to linear programming. \red{Specify.}
Suppose a decision procedure for $n-1$ is available, we give one for $n$.

The idea is use the equivalence given by Theorem~\ref{thm:locglob} and decide the Conditions~(1) and (2).
By Lemma~\ref{lem:decr}, Condition~(1) of Theorem~\ref{thm:locglob} is decidable.
For Condition~(2), it is equivalent to Condition~(2') in Proposition~\ref{prop:inftoshift}, and consequently equivalent to Condition~(2'') in Lemma~\ref{lem:shifttozero}. 

For each $P \in \mP$, enumerate all $\balpha_{P, Q}$ (there are finitely many of them by definition).
For each $\balpha_{P, Q}$ we check whether Equation~\eqref{eq:conddouble} is satisfied.
If Equation~\eqref{eq:conddouble} is satisfied, denote $I' \coloneqq \{i \in I \mid \alpha_{P, Q, i} = \min_{j \in J} \alpha_{P, Q, j}\}, J' \coloneqq \left(O_{v_P} \cup J\right)$; and we proceed to check whether there exists $\bff \in \init_{v_P, \balpha_{P, Q}}^0(\mM) \cap \left(\A_{n-1}^+\right)^K$ satisfying Condition~\eqref{eq:conddouble2}.
This check is done in the following way.
Note that by Lemma~\ref{lem:in0gen}, the set $\mM^0 \coloneqq \init_{v_P, \balpha_{P, Q}}^0(\mM)$ is the $\A_{n-1}$-module generated by $\init_{v_P, \balpha_{P, Q}}^0(\bg_j), j = 1, \ldots, m$.
Using the induction hypothesis on $\mM^0$, $J'$ and $I'$, we can decide whether it contains an element $\bff^0 \in \left(\A_{n-1}^+\right)^K$ satisfying
    \[
        \left(O_{w} \cup J'\right) \cap M_{w}(I', \init_{v_P}(\bff^0)) \neq \emptyset \quad \text{ for every $w \perp v_P$}.
    \]

Condition~(2) of Theorem~\ref{thm:locglob} is satisfied if and only if for every $P \in \mP$ there exist some $\balpha_{P, Q}$ and $\bff \in \init_{v_P, \balpha_{P, Q}}^0(\mM) \cap \left(\A_{n-1}^+\right)^K$ satisfying Conditions~\eqref{eq:conddouble} and \eqref{eq:conddouble2}.
Hence Condition~(2) of Theorem~\ref{thm:locglob} is also decidable.
We conclude the proof by the equivalence given by Theorem~\ref{thm:locglob}.
\end{proof}

\begin{example}
Suppose $n = 3$, $K = 1$ and $g = X_1 X_2 X_3 + X_2^2 X_3 + 1$.
Let $v = (1, 1, \sqrt{2})^{\top}$,
we can define 
\[
A = 
\begin{pmatrix}
    1 & 0 & 0 \\
    1 & 1 & 0 \\
    0 & 0 & 1 \\
\end{pmatrix}.
\]
We have $A^{-\top} v = (0, 1, \sqrt{2})$ where $1$ and $\sqrt{2}$ are $\Q$-linearly independent.
So $d = 1$.
The corresponding coordinate change is 
\[
\varphi_A \colon X_1 \mapsto X_1 X_2, X_2 \mapsto X_2, X_3 \mapsto X_3.
\]
Then $\varphi_A(g) = X_1 X_2^2 X_3 + X_2^2 X_3 + 1$.
We indeed have $\init_{(0, 1, \sqrt{2})^{\top}}(\varphi_A(g)) = X_1 X_2^2 X_3 + X_2^2 X_3 = X_2^2 X_3 \cdot (X_1 + 1)$.
So $\init_{v, 0}^{A, d}(g) = X_1 + 1$.

We verify the consistency of the variable change.
Indeed, $\init_v(g) = X_1 X_2 X_3 + X_2^2 X_3$, so $\varphi_A(\init_v(g)) = X_1 X_2^2 X_3 + X_2^2 X_3 = \init_{A^{-\top} v}(\varphi_A(g))$.
\end{example}
